Measurement of ${\mathcal B}$($B_s \rightarrow D_s X$) with $B_s$ Semileptonic Tagging

We report the first direct measurement of the inclusive branching fraction ${\mathcal B}(B_s \rightarrow D_s X)$ via $B_s$ tagging in $e^+e^-\to\Upsilon$(5S) events. Tagging is accomplished through a partial reconstruction of semileptonic decays $B_s \rightarrow D_s X \ell \nu$, where $X$ denotes unreconstructed additional hadrons or photons and $\ell$ is an electron or muon. With 121.4 fb$^{-1}$ of data collected at the $\Upsilon$(5S) resonance by the Belle detector at the KEKB asymmetric-energy $e^+ e^-$ collider, we obtain ${\mathcal B}(B_s \rightarrow D_s X)$ = $(60.2 \pm 5.8 \pm 2.3)$\%, where the first uncertainty is statistical and the second is systematic.

==> pub544.tex <==
%%% Paper:    Bs -> Ds X
%%% Journal:  Physical Review D
%%% Contacts: B. Wang (wang@mpp.mpg.de)
%%%           K. Kinoshita (kay.kinoshita@uc.edu)
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{author} to insert this material into your latex file.
%%%%% Force institutions to appear in alphabetical order when typeset.
\noaffiliation
\affiliation{University of the Basque Country UPV/EHU, 48080 Bilbao}
\affiliation{Beihang University, Beijing 100191}
%%%\affiliation{University of Bonn, 53115 Bonn}
\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}
\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague}
%%%\affiliation{Chiba University, Chiba 263-8522}
\affiliation{Chonnam National University, Kwangju 660-701}
\affiliation{University of Cincinnati, Cincinnati, Ohio 45221}
\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg}
%%%\affiliation{Duke University, Durham, North Carolina 27708}
%%%\affiliation{University of Florida, Gainesville, Florida 32611}
%%%\affiliation{Department of Physics, Fu Jen Catholic University, Taipei 24205}
\affiliation{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443}
\affiliation{Justus-Liebig-Universit\"at Gie\ss{}en, 35392 Gie\ss{}en}
%%%\affiliation{Gifu University, Gifu 501-1193}
\affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen}
\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193}
\affiliation{Gyeongsang National University, Chinju 660-701}
\affiliation{Hanyang University, Seoul 133-791}
\affiliation{University of Hawaii, Honolulu, Hawaii 96822}
\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}
\affiliation{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}
\affiliation{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich}
%%%\affiliation{Hiroshima Institute of Technology, Hiroshima 731-5193}
\affiliation{IKERBASQUE, Basque Foundation for Science, 48013 Bilbao}
%%%\affiliation{University of Illinois at Urbana-Champaign, Urbana, Illinois 61801}
\affiliation{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306}
\affiliation{Indian Institute of Technology Bhubaneswar, Satya Nagar 751007}
\affiliation{Indian Institute of Technology Guwahati, Assam 781039}
\affiliation{Indian Institute of Technology Hyderabad, Telangana 502285}
\affiliation{Indian Institute of Technology Madras, Chennai 600036}
%%%\affiliation{Indiana University, Bloomington, Indiana 47408}
\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049}
\affiliation{Institute of High Energy Physics, Vienna 1050}
\affiliation{Institute for High Energy Physics, Protvino 142281}
%%%\affiliation{Institute of Mathematical Sciences, Chennai 600113}
\affiliation{INFN - Sezione di Napoli, 80126 Napoli}
\affiliation{INFN - Sezione di Torino, 10125 Torino}
\affiliation{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195}
\affiliation{J. Stefan Institute, 1000 Ljubljana}
%%%\affiliation{Kanagawa University, Yokohama 221-8686}
\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe}
%%%\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583}
\affiliation{Kennesaw State University, Kennesaw, Georgia 30144}
\affiliation{King Abdulaziz City for Science and Technology, Riyadh 11442}
%%%\affiliation{Department of Physics, Faculty of Science, King Abdulaziz University, Jeddah 21589}
%%%\affiliation{Kitasato University, Sagamihara 252-0373}
\affiliation{Korea Institute of Science and Technology Information, Daejeon 305-806}
\affiliation{Korea University, Seoul 136-713}
%%%\affiliation{Kyoto University, Kyoto 606-8502}
\affiliation{Kyungpook National University, Daegu 702-701}
\affiliation{LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'{e} Paris-Saclay, Orsay}
\affiliation{\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne 1015}
\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}
%%%\affiliation{Liaoning Normal University, Dalian 116029}
\affiliation{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana}
\affiliation{Ludwig Maximilians University, 80539 Munich}
\affiliation{Luther College, Decorah, Iowa 52101}
%%%\affiliation{Malaviya National Institute of Technology Jaipur, Jaipur 302017}
%%%\affiliation{University of Malaya, 50603 Kuala Lumpur}
\affiliation{University of Maribor, 2000 Maribor}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen}
\affiliation{School of Physics, University of Melbourne, Victoria 3010}
\affiliation{University of Mississippi, University, Mississippi 38677}
\affiliation{University of Miyazaki, Miyazaki 889-2192}
%%%\affiliation{Moscow Physical Engineering Institute, Moscow 115409}
\affiliation{Moscow Institute of Physics and Technology, Moscow Region 141700}
\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602}
%%%\affiliation{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602}
\affiliation{Universit\`{a} di Napoli Federico II, 80055 Napoli}
%%%\affiliation{Nara University of Education, Nara 630-8528}
\affiliation{Nara Women's University, Nara 630-8506}
\affiliation{National Central University, Chung-li 32054}
\affiliation{National United University, Miao Li 36003}
\affiliation{Department of Physics, National Taiwan University, Taipei 10617}
\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342}
\affiliation{Nippon Dental University, Niigata 951-8580}
\affiliation{Niigata University, Niigata 950-2181}
%%%\affiliation{University of Nova Gorica, 5000 Nova Gorica}
\affiliation{Novosibirsk State University, Novosibirsk 630090}
\affiliation{Osaka City University, Osaka 558-8585}
%%%\affiliation{Osaka University, Osaka 565-0871}
\affiliation{Pacific Northwest National Laboratory, Richland, Washington 99352}
\affiliation{Panjab University, Chandigarh 160014}
\affiliation{Peking University, Beijing 100871}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260}
%%%\affiliation{Punjab Agricultural University, Ludhiana 141004}
%%%\affiliation{Research Center for Electron Photon Science, Tohoku University, Sendai 980-8578}
%%%\affiliation{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047}
\affiliation{Theoretical Research Division, Nishina Center, RIKEN, Saitama 351-0198}
%%%\affiliation{RIKEN BNL Research Center, Upton, New York 11973}
%%%\affiliation{Saga University, Saga 840-8502}
\affiliation{University of Science and Technology of China, Hefei 230026}
\affiliation{Seoul National University, Seoul 151-742}
%%%\affiliation{Shinshu University, Nagano 390-8621}
\affiliation{Showa Pharmaceutical University, Tokyo 194-8543}
\affiliation{Soongsil University, Seoul 156-743}
%%%\affiliation{University of South Carolina, Columbia, South Carolina 29208}
%%%\affiliation{Stefan Meyer Institute for Subatomic Physics, Vienna 1090}
\affiliation{Sungkyunkwan University, Suwon 440-746}
\affiliation{School of Physics, University of Sydney, New South Wales 2006}
\affiliation{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451}
\affiliation{Tata Institute of Fundamental Research, Mumbai 400005}
%%%\affiliation{Excellence Cluster Universe, Technische Universit\"at M\"unchen, 85748 Garching}
%%%\affiliation{Department of Physics, Technische Universit\"at M\"unchen, 85748 Garching}
\affiliation{Toho University, Funabashi 274-8510}
%%%\affiliation{Tohoku Gakuin University, Tagajo 985-8537}
\affiliation{Department of Physics, Tohoku University, Sendai 980-8578}
\affiliation{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032}
\affiliation{Department of Physics, University of Tokyo, Tokyo 113-0033}
%%%\affiliation{Tokyo Institute of Technology, Tokyo 152-8550}
\affiliation{Tokyo Metropolitan University, Tokyo 192-0397}
%%%\affiliation{Tokyo University of Agriculture and Technology, Tokyo 184-8588}
%%%\affiliation{Utkal University, Bhubaneswar 751004}
\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061}
\affiliation{Wayne State University, Detroit, Michigan 48202}
\affiliation{Yamagata University, Yamagata 990-8560}
\affiliation{Yonsei University, Seoul 120-749}
% \author{A.~Abdesselam}\affiliation{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451} % Tabuk
% \author{I.~Adachi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{K.~Adamczyk}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
% \author{J.~K.~Ahn}\affiliation{Korea University, Seoul 136-713} % Korea
  \author{B.~Wang}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221}  % MPI, Cincinnati
  \author{K.~Kinoshita}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
  \author{H.~Aihara}\affiliation{Department of Physics, University of Tokyo, Tokyo 113-0033} % Tokyo
% \author{S.~Al~Said}\affiliation{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451}\affiliation{Department of Physics, Faculty of Science, King Abdulaziz University, Jeddah 21589} % Tabuk
% \author{K.~Arinstein}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{Y.~Arita}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
  \author{D.~M.~Asner}\affiliation{Brookhaven National Laboratory, Upton, New York 11973} % BNL
% \author{H.~Atmacan}\affiliation{University of South Carolina, Columbia, South Carolina 29208} % SouthCarolina
% \author{V.~Aulchenko}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{T.~Aushev}\affiliation{Moscow Institute of Physics and Technology, Moscow Region 141700} % MIPT
  \author{R.~Ayad}\affiliation{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451} % Tabuk
% \author{T.~Aziz}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005} % Tata
  \author{V.~Babu}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
  \author{I.~Badhrees}\affiliation{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451}\affiliation{King Abdulaziz City for Science and Technology, Riyadh 11442} % Tabuk
% \author{S.~Bahinipati}\affiliation{Indian Institute of Technology Bhubaneswar, Satya Nagar 751007} % IITB
  \author{A.~M.~Bakich}\affiliation{School of Physics, University of Sydney, New South Wales 2006} % Sydney
% \author{Y.~Ban}\affiliation{Peking University, Beijing 100871} % Peking
% \author{V.~Bansal}\affiliation{Pacific Northwest National Laboratory, Richland, Washington 99352} % PNNL
% \author{E.~Barberio}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
% \author{M.~Barrett}\affiliation{Wayne State University, Detroit, Michigan 48202} % WayneState
% \author{W.~Bartel}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
  \author{P.~Behera}\affiliation{Indian Institute of Technology Madras, Chennai 600036} % IITM
  \author{C.~Bele\~{n}o}\affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen} % Goettingen
% \author{K.~Belous}\affiliation{Institute for High Energy Physics, Protvino 142281} % Protvino
  \author{J.~Bennett}\affiliation{University of Mississippi, University, Mississippi 38677} % Mississippi
% \author{M.~Berger}\affiliation{Stefan Meyer Institute for Subatomic Physics, Vienna 1090} % Vienna
% \author{F.~Bernlochner}\affiliation{University of Bonn, 53115 Bonn} % Bonn
  \author{M.~Bessner}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{D.~Besson}\affiliation{Moscow Physical Engineering Institute, Moscow 115409} % MEPhI
  \author{V.~Bhardwaj}\affiliation{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306} % IISERM
% \author{B.~Bhuyan}\affiliation{Indian Institute of Technology Guwahati, Assam 781039} % IITG
  \author{T.~Bilka}\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague} % Charles
  \author{J.~Biswal}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
% \author{T.~Bloomfield}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{A.~Bobrov}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{A.~Bondar}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{G.~Bonvicini}\affiliation{Wayne State University, Detroit, Michigan 48202} % WayneState
  \author{A.~Bozek}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
  \author{M.~Bra\v{c}ko}\affiliation{University of Maribor, 2000 Maribor}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
% \author{N.~Braun}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{F.~Breibeck}\affiliation{Institute of High Energy Physics, Vienna 1050} % Vienna
  \author{T.~E.~Browder}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{M.~Campajola}\affiliation{INFN - Sezione di Napoli, 80126 Napoli}\affiliation{Universit\`{a} di Napoli Federico II, 80055 Napoli} % Napoli
  \author{L.~Cao}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{G.~Caria}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{D.~\v{C}ervenkov}\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague} % Charles
% \author{M.-C.~Chang}\affiliation{Department of Physics, Fu Jen Catholic University, Taipei 24205} % FuJen
% \author{P.~Chang}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{Y.~Chao}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{R.~Cheaib}\affiliation{University of Mississippi, University, Mississippi 38677} % Mississippi
% \author{V.~Chekelian}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
  \author{A.~Chen}\affiliation{National Central University, Chung-li 32054} % NCU
% \author{K.-F.~Chen}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{B.~G.~Cheon}\affiliation{Hanyang University, Seoul 133-791} % Hanyang
  \author{K.~Chilikin}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % Lebedev
% \author{R.~Chistov}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}\affiliation{Moscow Physical Engineering Institute, Moscow 115409} % Lebedev
  \author{H.~E.~Cho}\affiliation{Hanyang University, Seoul 133-791} % Hanyang
  \author{K.~Cho}\affiliation{Korea Institute of Science and Technology Information, Daejeon 305-806} % KISTI
% \author{V.~Chobanova}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
  \author{S.-K.~Choi}\affiliation{Gyeongsang National University, Chinju 660-701} % Gyeongsang
  \author{Y.~Choi}\affiliation{Sungkyunkwan University, Suwon 440-746} % Sungkyunkwan
% \author{S.~Choudhury}\affiliation{Indian Institute of Technology Hyderabad, Telangana 502285} % IITH
  \author{D.~Cinabro}\affiliation{Wayne State University, Detroit, Michigan 48202} % WayneState
% \author{J.~Crnkovic}\affiliation{University of Illinois at Urbana-Champaign, Urbana, Illinois 61801} % UIUC
  \author{S.~Cunliffe}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
% \author{T.~Czank}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
% \author{M.~Danilov}\affiliation{Moscow Physical Engineering Institute, Moscow 115409}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % Lebedev
  \author{N.~Dash}\affiliation{Indian Institute of Technology Bhubaneswar, Satya Nagar 751007} % IITB
% \author{G.~De~Nardo}\affiliation{INFN - Sezione di Napoli, 80126 Napoli}\affiliation{Universit\`{a} di Napoli Federico II, 80055 Napoli} % Napoli
  \author{F.~Di~Capua}\affiliation{INFN - Sezione di Napoli, 80126 Napoli}\affiliation{Universit\`{a} di Napoli Federico II, 80055 Napoli} % Napoli
  \author{S.~Di~Carlo}\affiliation{LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'{e} Paris-Saclay, Orsay} % LAL
% \author{J.~Dingfelder}\affiliation{University of Bonn, 53115 Bonn} % Bonn
  \author{Z.~Dole\v{z}al}\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague} % Charles
% \author{T.~V.~Dong}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{D.~Dossett}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
% \author{Z.~Dr\'asal}\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague} % Charles
% \author{A.~Drutskoy}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}\affiliation{Moscow Physical Engineering Institute, Moscow 115409} % Lebedev
% \author{S.~Dubey}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{D.~Dutta}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005} % Tata
  \author{S.~Eidelman}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % BINP
  \author{D.~Epifanov}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{J.~E.~Fast}\affiliation{Pacific Northwest National Laboratory, Richland, Washington 99352} % PNNL
% \author{M.~Feindt}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
  \author{T.~Ferber}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
% \author{A.~Frey}\affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen} % Goettingen
% \author{O.~Frost}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
  \author{B.~G.~Fulsom}\affiliation{Pacific Northwest National Laboratory, Richland, Washington 99352} % PNNL
  \author{R.~Garg}\affiliation{Panjab University, Chandigarh 160014} % Panjab
  \author{V.~Gaur}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
% \author{N.~Gabyshev}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{A.~Garmash}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{M.~Gelb}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{J.~Gemmler}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{D.~Getzkow}\affiliation{Justus-Liebig-Universit\"at Gie\ss{}en, 35392 Gie\ss{}en} % Giessen
% \author{F.~Giordano}\affiliation{University of Illinois at Urbana-Champaign, Urbana, Illinois 61801} % UIUC
  \author{A.~Giri}\affiliation{Indian Institute of Technology Hyderabad, Telangana 502285} % IITH
  \author{P.~Goldenzweig}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{B.~Golob}\affiliation{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
% \author{D.~Greenwald}\affiliation{Department of Physics, Technische Universit\"at M\"unchen, 85748 Garching} % TUM
% \author{M.~Grosse~Perdekamp}\affiliation{University of Illinois at Urbana-Champaign, Urbana, Illinois 61801}\affiliation{RIKEN BNL Research Center, Upton, New York 11973} % UIUC
% \author{J.~Grygier}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
  \author{Y.~Guan}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{E.~Guido}\affiliation{INFN - Sezione di Torino, 10125 Torino} % Torino
% \author{H.~Guo}\affiliation{University of Science and Technology of China, Hefei 230026} % USTC
% \author{J.~Haba}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{P.~Hamer}\affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen} % Goettingen
% \author{K.~Hara}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{T.~Hara}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{O.~Hartbrich}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{Y.~Hasegawa}\affiliation{Shinshu University, Nagano 390-8621} % Shinshu
% \author{J.~Hasenbusch}\affiliation{University of Bonn, 53115 Bonn} % Bonn
\author{K.~Hayasaka}\affiliation{Niigata University, Niigata 950-2181} % Niigata
  \author{H.~Hayashii}\affiliation{Nara Women's University, Nara 630-8506} % Nara
% \author{X.~H.~He}\affiliation{Peking University, Beijing 100871} % Peking
% \author{M.~Heck}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{M.~T.~Hedges}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{D.~Heffernan}\affiliation{Osaka University, Osaka 565-0871} % Osaka
% \author{M.~Heider}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{A.~Heller}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{T.~Higuchi}\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583} % IPMU
% \author{S.~Hirose}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
% \author{T.~Horiguchi}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
% \author{Y.~Hoshi}\affiliation{Tohoku Gakuin University, Tagajo 985-8537} % TohokuGakuin
% \author{K.~Hoshina}\affiliation{Tokyo University of Agriculture and Technology, Tokyo 184-8588} % TUAT
  \author{W.-S.~Hou}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{Y.~B.~Hsiung}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{C.-L.~Hsu}\affiliation{School of Physics, University of Sydney, New South Wales 2006} % Sydney
% \author{K.~Huang}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{M.~Huschle}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{Y.~Igarashi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{T.~Iijima}\affiliation{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
% \author{M.~Imamura}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
  \author{K.~Inami}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
% \author{G.~Inguglia}\affiliation{Institute of High Energy Physics, Vienna 1050} % Vienna
  \author{A.~Ishikawa}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{K.~Itagaki}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
% \author{R.~Itoh}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{M.~Iwasaki}\affiliation{Osaka City University, Osaka 558-8585} % OsakaCity
  \author{Y.~Iwasaki}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{S.~Iwata}\affiliation{Tokyo Metropolitan University, Tokyo 192-0397} % TMU
% \author{W.~W.~Jacobs}\affiliation{Indiana University, Bloomington, Indiana 47408} % Indiana
% \author{I.~Jaegle}\affiliation{University of Florida, Gainesville, Florida 32611} % Florida
% \author{H.~B.~Jeon}\affiliation{Kyungpook National University, Daegu 702-701} % Kyungpook
  \author{S.~Jia}\affiliation{Beihang University, Beijing 100191} % Beihang
  \author{Y.~Jin}\affiliation{Department of Physics, University of Tokyo, Tokyo 113-0033} % Tokyo
  \author{D.~Joffe}\affiliation{Kennesaw State University, Kennesaw, Georgia 30144} % Kennesaw
% \author{M.~Jones}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{C.~W.~Joo}\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583} % IPMU
  \author{K.~K.~Joo}\affiliation{Chonnam National University, Kwangju 660-701} % Chonnam
% \author{T.~Julius}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
% \author{J.~Kahn}\affiliation{Ludwig Maximilians University, 80539 Munich} % LMU
% \author{H.~Kakuno}\affiliation{Tokyo Metropolitan University, Tokyo 192-0397} % TMU
  \author{A.~B.~Kaliyar}\affiliation{Indian Institute of Technology Madras, Chennai 600036} % IITM
% \author{J.~H.~Kang}\affiliation{Yonsei University, Seoul 120-749} % Yonsei
  \author{K.~H.~Kang}\affiliation{Kyungpook National University, Daegu 702-701} % Kyungpook
% \author{P.~Kapusta}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
  \author{G.~Karyan}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
% \author{S.~U.~Kataoka}\affiliation{Nara University of Education, Nara 630-8528} % NUE
% \author{E.~Kato}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
% \author{Y.~Kato}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
% \author{P.~Katrenko}\affiliation{Moscow Institute of Physics and Technology, Moscow Region 141700}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % Lebedev
% \author{H.~Kawai}\affiliation{Chiba University, Chiba 263-8522} % Chiba
% \author{T.~Kawasaki}\affiliation{Kitasato University, Sagamihara 252-0373} % Kitasato
% \author{T.~Keck}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{H.~Kichimi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
  \author{C.~Kiesling}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
% \author{B.~H.~Kim}\affiliation{Seoul National University, Seoul 151-742} % Seoul
% \author{C.~H.~Kim}\affiliation{Hanyang University, Seoul 133-791} % Hanyang
  \author{D.~Y.~Kim}\affiliation{Soongsil University, Seoul 156-743} % Soongsil
% \author{H.~J.~Kim}\affiliation{Kyungpook National University, Daegu 702-701} % Kyungpook
% \author{H.-J.~Kim}\affiliation{Yonsei University, Seoul 120-749} % Yonsei
% \author{J.~B.~Kim}\affiliation{Korea University, Seoul 136-713} % Korea
  \author{K.~T.~Kim}\affiliation{Korea University, Seoul 136-713} % Korea
  \author{S.~H.~Kim}\affiliation{Hanyang University, Seoul 133-791} % Hanyang
% \author{S.~K.~Kim}\affiliation{Seoul National University, Seoul 151-742} % Seoul
% \author{Y.~J.~Kim}\affiliation{Korea University, Seoul 136-713} % Korea
% \author{T.~D.~Kimmel}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
% \author{H.~Kindo}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{C.~Kleinwort}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
% \author{J.~Klucar}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
% \author{N.~Kobayashi}\affiliation{Tokyo Institute of Technology, Tokyo 152-8550} % NPC
  \author{P.~Kody\v{s}}\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague} % Charles
% \author{Y.~Koga}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
% \author{T.~Konno}\affiliation{Kitasato University, Sagamihara 252-0373} % Kitasato
  \author{S.~Korpar}\affiliation{University of Maribor, 2000 Maribor}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
  \author{D.~Kotchetkov}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{R.~T.~Kouzes}\affiliation{Pacific Northwest National Laboratory, Richland, Washington 99352} % PNNL
  \author{P.~Kri\v{z}an}\affiliation{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
  \author{R.~Kroeger}\affiliation{University of Mississippi, University, Mississippi 38677} % Mississippi
% \author{J.-F.~Krohn}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{P.~Krokovny}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{B.~Kronenbitter}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
  \author{T.~Kuhr}\affiliation{Ludwig Maximilians University, 80539 Munich} % LMU
% \author{R.~Kulasiri}\affiliation{Kennesaw State University, Kennesaw, Georgia 30144} % Kennesaw
% \author{R.~Kumar}\affiliation{Punjab Agricultural University, Ludhiana 141004} % Punjab
% \author{T.~Kumita}\affiliation{Tokyo Metropolitan University, Tokyo 192-0397} % TMU
% \author{E.~Kurihara}\affiliation{Chiba University, Chiba 263-8522} % Chiba
% \author{Y.~Kuroki}\affiliation{Osaka University, Osaka 565-0871} % Osaka
  \author{A.~Kuzmin}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{P.~Kvasni\v{c}ka}\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague} % Charles
  \author{Y.-J.~Kwon}\affiliation{Yonsei University, Seoul 120-749} % Yonsei
% \author{Y.-T.~Lai}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{K.~Lalwani}\affiliation{Malaviya National Institute of Technology Jaipur, Jaipur 302017} % MNIT
  \author{J.~S.~Lange}\affiliation{Justus-Liebig-Universit\"at Gie\ss{}en, 35392 Gie\ss{}en} % Giessen
  \author{I.~S.~Lee}\affiliation{Hanyang University, Seoul 133-791} % Hanyang
% \author{J.~K.~Lee}\affiliation{Seoul National University, Seoul 151-742} % Seoul
  \author{J.~Y.~Lee}\affiliation{Seoul National University, Seoul 151-742} % Seoul
  \author{S.~C.~Lee}\affiliation{Kyungpook National University, Daegu 702-701} % Kyungpook
% \author{M.~Leitgab}\affiliation{University of Illinois at Urbana-Champaign, Urbana, Illinois 61801}\affiliation{RIKEN BNL Research Center, Upton, New York 11973} % UIUC
% \author{R.~Leitner}\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague} % Charles
% \author{D.~Levit}\affiliation{Department of Physics, Technische Universit\"at M\"unchen, 85748 Garching} % TUM
% \author{P.~Lewis}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{C.~H.~Li}\affiliation{Liaoning Normal University, Dalian 116029} % LNNU
% \author{H.~Li}\affiliation{Indiana University, Bloomington, Indiana 47408} % Indiana
  \author{L.~K.~Li}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049} % IHEP
% \author{Y.~Li}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
  \author{Y.~B.~Li}\affiliation{Peking University, Beijing 100871} % Peking
  \author{L.~Li~Gioi}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
  \author{J.~Libby}\affiliation{Indian Institute of Technology Madras, Chennai 600036} % IITM
  \author{K.~Lieret}\affiliation{Ludwig Maximilians University, 80539 Munich} % LMU
% \author{A.~Limosani}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
% \author{Z.~Liptak}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{C.~Liu}\affiliation{University of Science and Technology of China, Hefei 230026} % USTC
% \author{Y.~Liu}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
  \author{D.~Liventsev}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % VPI
% \author{A.~Loos}\affiliation{University of South Carolina, Columbia, South Carolina 29208} % SouthCarolina
% \author{R.~Louvot}\affiliation{\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne 1015} % Lausanne
% \author{P.-C.~Lu}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{M.~Lubej}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
  \author{T.~Luo}\affiliation{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443} % Fudan
  \author{J.~MacNaughton}\affiliation{University of Miyazaki, Miyazaki 889-2192} % NPC
  \author{C.~MacQueen}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{M.~Masuda}\affiliation{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032} % NPC
  \author{T.~Matsuda}\affiliation{University of Miyazaki, Miyazaki 889-2192} % NPC
  \author{D.~Matvienko}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % BINP
% \author{J.~T.~McNeil}\affiliation{University of Florida, Gainesville, Florida 32611} % Florida
  \author{M.~Merola}\affiliation{INFN - Sezione di Napoli, 80126 Napoli}\affiliation{Universit\`{a} di Napoli Federico II, 80055 Napoli} % Napoli
% \author{F.~Metzner}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{Y.~Mikami}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
\author{K.~Miyabayashi}\affiliation{Nara Women's University, Nara 630-8506} % Nara
% \author{Y.~Miyachi}\affiliation{Yamagata University, Yamagata 990-8560} % NPC
% \author{H.~Miyake}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{H.~Miyata}\affiliation{Niigata University, Niigata 950-2181} % Niigata
% \author{Y.~Miyazaki}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
  \author{R.~Mizuk}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}\affiliation{Moscow Institute of Physics and Technology, Moscow Region 141700} % Lebedev
  \author{G.~B.~Mohanty}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005} % Tata
% \author{S.~Mohanty}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005}\affiliation{Utkal University, Bhubaneswar 751004} % Tata
% \author{H.~K.~Moon}\affiliation{Korea University, Seoul 136-713} % Korea
% \author{T.~J.~Moon}\affiliation{Seoul National University, Seoul 151-742} % Seoul
% \author{T.~Mori}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
% \author{T.~Morii}\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583} % IPMU
% \author{H.-G.~Moser}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
% \author{M.~Mrvar}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
% \author{T.~M\"uller}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{N.~Muramatsu}\affiliation{Research Center for Electron Photon Science, Tohoku University, Sendai 980-8578} % NPC
  \author{R.~Mussa}\affiliation{INFN - Sezione di Torino, 10125 Torino} % Torino
% \author{Y.~Nagasaka}\affiliation{Hiroshima Institute of Technology, Hiroshima 731-5193} % Hiroshima
% \author{Y.~Nakahama}\affiliation{Department of Physics, University of Tokyo, Tokyo 113-0033} % Tokyo
% \author{I.~Nakamura}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{K.~R.~Nakamura}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{E.~Nakano}\affiliation{Osaka City University, Osaka 558-8585} % OsakaCity
% \author{H.~Nakano}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
% \author{T.~Nakano}\affiliation{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047} % NPC
  \author{M.~Nakao}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{H.~Nakayama}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{H.~Nakazawa}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{T.~Nanut}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
  \author{K.~J.~Nath}\affiliation{Indian Institute of Technology Guwahati, Assam 781039} % IITG
% \author{Z.~Natkaniec}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
  \author{M.~Nayak}\affiliation{Wayne State University, Detroit, Michigan 48202}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % WayneState
% \author{K.~Neichi}\affiliation{Tohoku Gakuin University, Tagajo 985-8537} % TohokuGakuin
% \author{C.~Ng}\affiliation{Department of Physics, University of Tokyo, Tokyo 113-0033} % Tokyo
% \author{C.~Niebuhr}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
% \author{M.~Niiyama}\affiliation{Kyoto University, Kyoto 606-8502} % NPC
  \author{N.~K.~Nisar}\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260} % Pittsburgh
  \author{S.~Nishida}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{K.~Nishimura}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{O.~Nitoh}\affiliation{Tokyo University of Agriculture and Technology, Tokyo 184-8588} % TUAT
% \author{A.~Ogawa}\affiliation{RIKEN BNL Research Center, Upton, New York 11973} % RIKEN
% \author{K.~Ogawa}\affiliation{Niigata University, Niigata 950-2181} % Niigata
  \author{S.~Ogawa}\affiliation{Toho University, Funabashi 274-8510} % Toho
% \author{T.~Ohshima}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
% \author{S.~Okuno}\affiliation{Kanagawa University, Yokohama 221-8686} % Kanagawa
% \author{S.~L.~Olsen}\affiliation{Gyeongsang National University, Chinju 660-701} % Gyeongsang
  \author{H.~Ono}\affiliation{Nippon Dental University, Niigata 951-8580}\affiliation{Niigata University, Niigata 950-2181} % NihonDental
% \author{Y.~Ono}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
  \author{Y.~Onuki}\affiliation{Department of Physics, University of Tokyo, Tokyo 113-0033} % Tokyo
% \author{W.~Ostrowicz}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
% \author{C.~Oswald}\affiliation{University of Bonn, 53115 Bonn} % Bonn
% \author{H.~Ozaki}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{P.~Pakhlov}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}\affiliation{Moscow Physical Engineering Institute, Moscow 115409} % Lebedev
  \author{G.~Pakhlova}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}\affiliation{Moscow Institute of Physics and Technology, Moscow Region 141700} % Lebedev
  \author{B.~Pal}\affiliation{Brookhaven National Laboratory, Upton, New York 11973} % BNL
  \author{T.~Pang}\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260} % Pittsburgh
% \author{E.~Panzenb\"ock}\affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen}\affiliation{Nara Women's University, Nara 630-8506} % Goettingen
  \author{S.~Pardi}\affiliation{INFN - Sezione di Napoli, 80126 Napoli} % Napoli
% \author{C.-S.~Park}\affiliation{Yonsei University, Seoul 120-749} % Yonsei
% \author{C.~W.~Park}\affiliation{Sungkyunkwan University, Suwon 440-746} % Sungkyunkwan
  \author{H.~Park}\affiliation{Kyungpook National University, Daegu 702-701} % Kyungpook
% \author{K.~S.~Park}\affiliation{Sungkyunkwan University, Suwon 440-746} % Sungkyunkwan
  \author{S.-H.~Park}\affiliation{Yonsei University, Seoul 120-749} % Yonsei
% \author{S.~Patra}\affiliation{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306} % IISERM
% \author{S.~Paul}\affiliation{Department of Physics, Technische Universit\"at M\"unchen, 85748 Garching} % TUM
% \author{I.~Pavelkin}\affiliation{Moscow Institute of Physics and Technology, Moscow Region 141700} % MIPT
  \author{T.~K.~Pedlar}\affiliation{Luther College, Decorah, Iowa 52101} % Luther
% \author{T.~Peng}\affiliation{University of Science and Technology of China, Hefei 230026} % USTC
% \author{L.~Pes\'{a}ntez}\affiliation{University of Bonn, 53115 Bonn} % Bonn
  \author{R.~Pestotnik}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
% \author{M.~Peters}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{L.~E.~Piilonen}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
  \author{V.~Popov}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}\affiliation{Moscow Institute of Physics and Technology, Moscow Region 141700} % MIPT
% \author{K.~Prasanth}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005} % Tata
  \author{E.~Prencipe}\affiliation{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich} % Juelich
 \author{M.~Prim}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{K.~Prothmann}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen}\affiliation{Excellence Cluster Universe, Technische Universit\"at M\"unchen, 85748 Garching} % MPI
% \author{M.~V.~Purohit}\affiliation{University of South Carolina, Columbia, South Carolina 29208} % SouthCarolina
% \author{A.~Rabusov}\affiliation{Department of Physics, Technische Universit\"at M\"unchen, 85748 Garching} % TUM
% \author{J.~Rauch}\affiliation{Department of Physics, Technische Universit\"at M\"unchen, 85748 Garching} % TUM
% \author{B.~Reisert}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
% \author{P.~K.~Resmi}\affiliation{Indian Institute of Technology Madras, Chennai 600036} % IITM
% \author{E.~Ribe\v{z}l}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
  \author{M.~Ritter}\affiliation{Ludwig Maximilians University, 80539 Munich} % LMU
% \author{J.~Rorie}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{A.~Rostomyan}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
% \author{M.~Rozanska}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
% \author{S.~Rummel}\affiliation{Ludwig Maximilians University, 80539 Munich} % LMU
  \author{G.~Russo}\affiliation{Universit\`{a} di Napoli Federico II, 80055 Napoli} % Napoli
% \author{D.~Sahoo}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005} % Tata
% \author{H.~Sahoo}\affiliation{University of Mississippi, University, Mississippi 38677} % Mississippi
% \author{T.~Saito}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
% \author{Y.~Sakai}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{M.~Salehi}\affiliation{University of Malaya, 50603 Kuala Lumpur}\affiliation{Ludwig Maximilians University, 80539 Munich} % Malaya
  \author{S.~Sandilya}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{A.~Sangal}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{D.~Santel}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
  \author{L.~Santelj}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
  \author{T.~Sanuki}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
% \author{J.~Sasaki}\affiliation{Department of Physics, University of Tokyo, Tokyo 113-0033} % Tokyo
% \author{N.~Sasao}\affiliation{Kyoto University, Kyoto 606-8502} % Kyoto
% \author{Y.~Sato}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
  \author{V.~Savinov}\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260} % Pittsburgh
% \author{T.~Schl\"{u}ter}\affiliation{Ludwig Maximilians University, 80539 Munich} % LMU
  \author{O.~Schneider}\affiliation{\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne 1015} % Lausanne
  \author{G.~Schnell}\affiliation{University of the Basque Country UPV/EHU, 48080 Bilbao}\affiliation{IKERBASQUE, Basque Foundation for Science, 48013 Bilbao} % Bilbao
% \author{P.~Sch\"onmeier}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
% \author{M.~Schram}\affiliation{Pacific Northwest National Laboratory, Richland, Washington 99352} % PNNL
% \author{J.~Schueler}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{C.~Schwanda}\affiliation{Institute of High Energy Physics, Vienna 1050} % Vienna
 \author{A.~J.~Schwartz}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{B.~Schwenker}\affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen} % Goettingen
% \author{R.~Seidl}\affiliation{RIKEN BNL Research Center, Upton, New York 11973} % RIKEN
  \author{Y.~Seino}\affiliation{Niigata University, Niigata 950-2181} % Niigata
% \author{D.~Semmler}\affiliation{Justus-Liebig-Universit\"at Gie\ss{}en, 35392 Gie\ss{}en} % Giessen
  \author{K.~Senyo}\affiliation{Yamagata University, Yamagata 990-8560} % Yamagata
% \author{O.~Seon}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
% \author{I.~S.~Seong}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{M.~E.~Sevior}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
% \author{L.~Shang}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049} % IHEP
% \author{M.~Shapkin}\affiliation{Institute for High Energy Physics, Protvino 142281} % Protvino
  \author{V.~Shebalin}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{C.~P.~Shen}\affiliation{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443} % Fudan
% \author{T.-A.~Shibata}\affiliation{Tokyo Institute of Technology, Tokyo 152-8550} % NPC
% \author{H.~Shibuya}\affiliation{Toho University, Funabashi 274-8510} % Toho
% \author{S.~Shinomiya}\affiliation{Osaka University, Osaka 565-0871} % Osaka
  \author{J.-G.~Shiu}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{B.~Shwartz}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{A.~Sibidanov}\affiliation{School of Physics, University of Sydney, New South Wales 2006} % Sydney
% \author{F.~Simon}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
% \author{J.~B.~Singh}\affiliation{Panjab University, Chandigarh 160014} % Panjab
% \author{R.~Sinha}\affiliation{Institute of Mathematical Sciences, Chennai 600113} % IMSC
% \author{K.~Smith}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{A.~Sokolov}\affiliation{Institute for High Energy Physics, Protvino 142281} % Protvino
% \author{Y.~Soloviev}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
  \author{E.~Solovieva}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % Lebedev
% \author{S.~Stani\v{c}}\affiliation{University of Nova Gorica, 5000 Nova Gorica} % NovaGorica
  \author{M.~Stari\v{c}}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
% \author{M.~Steder}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
% \author{Z.~S.~Stottler}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
  \author{J.~F.~Strube}\affiliation{Pacific Northwest National Laboratory, Richland, Washington 99352} % PNNL
% \author{J.~Stypula}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
% \author{S.~Sugihara}\affiliation{Department of Physics, University of Tokyo, Tokyo 113-0033} % Tokyo
% \author{A.~Sugiyama}\affiliation{Saga University, Saga 840-8502} % Saga
% \author{M.~Sumihama}\affiliation{Gifu University, Gifu 501-1193} % NPC
% \author{K.~Sumisawa}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{T.~Sumiyoshi}\affiliation{Tokyo Metropolitan University, Tokyo 192-0397} % TMU
% \author{W.~Sutcliffe}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{K.~Suzuki}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
% \author{K.~Suzuki}\affiliation{Stefan Meyer Institute for Subatomic Physics, Vienna 1090} % Vienna
% \author{S.~Suzuki}\affiliation{Saga University, Saga 840-8502} % Saga
% \author{S.~Y.~Suzuki}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{Z.~Suzuki}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
% \author{H.~Takeichi}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
  \author{M.~Takizawa}\affiliation{Showa Pharmaceutical University, Tokyo 194-8543}\affiliation{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{Theoretical Research Division, Nishina Center, RIKEN, Saitama 351-0198} % NPC
% \author{U.~Tamponi}\affiliation{INFN - Sezione di Torino, 10125 Torino} % Torino
% \author{M.~Tanaka}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{S.~Tanaka}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{K.~Tanida}\affiliation{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195} % NPC
% \author{N.~Taniguchi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{Y.~Tao}\affiliation{University of Florida, Gainesville, Florida 32611} % Florida
% \author{G.~N.~Taylor}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{F.~Tenchini}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
% \author{Y.~Teramoto}\affiliation{Osaka City University, Osaka 558-8585} % OsakaCity
% \author{K.~Trabelsi}\affiliation{LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'{e} Paris-Saclay, Orsay} % LAL
% \author{T.~Tsuboyama}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{M.~Uchida}\affiliation{Tokyo Institute of Technology, Tokyo 152-8550} % NPC
% \author{I.~Ueda}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{S.~Uehara}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{T.~Uglov}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}\affiliation{Moscow Institute of Physics and Technology, Moscow Region 141700} % Lebedev
% \author{Y.~Unno}\affiliation{Hanyang University, Seoul 133-791} % Hanyang
  \author{S.~Uno}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{P.~Urquijo}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
% \author{Y.~Ushiroda}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{Y.~Usov}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{S.~E.~Vahsen}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{C.~Van~Hulse}\affiliation{University of the Basque Country UPV/EHU, 48080 Bilbao} % Bilbao
  \author{R.~Van~Tonder}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{P.~Vanhoefer}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI 
  \author{G.~Varner}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{K.~E.~Varvell}\affiliation{School of Physics, University of Sydney, New South Wales 2006} % Sydney
% \author{K.~Vervink}\affiliation{\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne 1015} % Lausanne
  \author{A.~Vinokurova}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{V.~Vorobyev}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % BINP
% \author{A.~Vossen}\affiliation{Duke University, Durham, North Carolina 27708} % Duke
% \author{M.~N.~Wagner}\affiliation{Justus-Liebig-Universit\"at Gie\ss{}en, 35392 Gie\ss{}en} % Giessen
  \author{E.~Waheed}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{C.~H.~Wang}\affiliation{National United University, Miao Li 36003} % NUU
  \author{M.-Z.~Wang}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
  \author{P.~Wang}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049} % IHEP
% \author{X.~L.~Wang}\affiliation{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443} % Fudan
% \author{M.~Watanabe}\affiliation{Niigata University, Niigata 950-2181} % Niigata
% \author{Y.~Watanabe}\affiliation{Kanagawa University, Yokohama 221-8686} % Kanagawa
% \author{S.~Watanuki}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
% \author{R.~Wedd}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
% \author{S.~Wehle}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
  \author{O.~Werbycka}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
% \author{E.~Widmann}\affiliation{Stefan Meyer Institute for Subatomic Physics, Vienna 1090} % Vienna
% \author{J.~Wiechczynski}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
% \author{K.~M.~Williams}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
  \author{E.~Won}\affiliation{Korea University, Seoul 136-713} % Korea
% \author{B.~D.~Yabsley}\affiliation{School of Physics, University of Sydney, New South Wales 2006} % Sydney
% \author{S.~Yamada}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{H.~Yamamoto}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
% \author{Y.~Yamashita}\affiliation{Nippon Dental University, Niigata 951-8580} % NihonDental
  \author{S.~B.~Yang}\affiliation{Korea University, Seoul 136-713} % Korea
% \author{S.~Yashchenko}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
  \author{H.~Ye}\affiliation{Deutsches Elektronen--Synchrotron, 22607 Hamburg} % DESY
% \author{J.~Yelton}\affiliation{University of Florida, Gainesville, Florida 32611} % Florida
% \author{J.~H.~Yin}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049} % IHEP
% \author{Y.~Yook}\affiliation{Yonsei University, Seoul 120-749} % Yonsei
% \author{C.~Z.~Yuan}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049} % IHEP
  \author{Y.~Yusa}\affiliation{Niigata University, Niigata 950-2181} % Niigata
% \author{S.~Zakharov}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}\affiliation{Moscow Institute of Physics and Technology, Moscow Region 141700} % MIPT
% \author{C.~C.~Zhang}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049} % IHEP
% \author{J.~Zhang}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049} % IHEP
% \author{L.~M.~Zhang}\affiliation{University of Science and Technology of China, Hefei 230026} % USTC
  \author{Z.~P.~Zhang}\affiliation{University of Science and Technology of China, Hefei 230026} % USTC
% \author{L.~Zhao}\affiliation{University of Science and Technology of China, Hefei 230026} % USTC
  \author{V.~Zhilich}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{V.~Zhukova}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % Lebedev
  \author{V.~Zhulanov}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{T.~Zivko}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
% \author{A.~Zupanc}\affiliation{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
% \author{N.~Zwahlen}\affiliation{\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne 1015} % Lausanne
\collaboration{The Belle Collaboration}

